Incorporating doubly resonant $W^\pm$ data in a global fit of SMEFT parameters to lift flat directions

We calculate the double pole contribution to two to four fermion scattering through $W^{\pm}$ currents at tree level in the Standard Model Effective Field Theory (SMEFT). We assume all fermions to be massless, $\rm U(3)^5$ flavour and $\rm CP$ symmetry. Using this result, we update the global constraint picture on SMEFT parameters including LEPII data on these charged current processes, and also include modifications to our fit procedure motivated by a companion paper focused on $W^{\pm}$ mass extractions. The fit reported is now to 177 observables and emphasises the need for a consistent inclusion of theoretical errors, and a consistent treatment of observables. Including charged current data lifts the two-fold degeneracy previously encountered in LEP (and lower energy) data, and allows us to set simultaneous constraints on 20 of 53 Wilson coefficients in the SMEFT, consistent with our assumptions. This allows the model independent inclusion of LEP data in SMEFT studies at LHC, which are projected into the SMEFT in a consistent fashion. We show how stronger constraints can be obtained by using some combinations of Wilson coefficients, when making assumptions on the UV completion of the Standard Model, or in an inconsistent analysis. We explain why strong bounds at the per-mille or sub-per-mille level on some combinations of Wilson coefficients in the Effective Lagrangian can be artificially enhanced in fits of this form in detail. This explains some of the different claims present in the literature.

==> TableWilsonUVren-1.tex <==
\begin{table}
\centering
\tabcolsep 4pt
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$C_i^G$ & $(1 \sigma,0)$ & $(1 \sigma, 0.1 \%)$ & $(1 \sigma, 0.3 \%)$   & $(1 \sigma, 0.5 \%)$ & $(1 \sigma, 1 \%)$  \\ 
\hline \hline
$\tilde{C}_{He} $ &$-0.11 \pm 1.6$&	$0.040 \pm 1.6$&	$0.18 \pm 1.7$&$0.31 \pm 1.8$&$0.35 \pm 2$\\
$\tilde{C}_{Hu}$ & $1.2 \pm 1.3$&	$1.1 \pm 1.3$&	$1.0 \pm 1.4$&$0.98 \pm 1.4$& $0.95 \pm 1.5$\\
$\tilde{C}_{Hd}$ &$-3.4 \pm 1.4$&	$-3.4 \pm 1.4$&	$-3.4 \pm 1.4$&$-3.4 \pm 1.4$&$-3.4 \pm 1.6$\\
$\tilde{C}_{Hl}^{(1)}$ &$0.032 \pm 0.82$&	$0.079 \pm 0.84$&		$0.23 \pm 0.90$&$0.30 \pm 0.96$&$0.32 \pm 1.1$\\
$\tilde{C}_{Hl}^{(3)}$ & $-0.33 \pm 3.0$&	$-0.22 \pm 3.0$&	 $0.13 \pm 3.1$& $0.33 \pm 3.3$&$0.36 \pm 3.5$\\
$\tilde{C}_{Hq}^{(1)}$ &$-0.048 \pm 0.32$&	$-0.057 \pm 0.32$&	$-0.085 \pm 0.33$& $-0.10 \pm 0.34$&$-0.11 \pm 0.37$\\
$\tilde{C}_{Hq}^{(3)}$ & $-0.71 \pm 3.0$&	$-0.58 \pm 3.0$&	$-0.19 \pm 3.2$&$0.018 \pm 3.3$&$0.052 \pm 3.5$\\
$\tilde{C}_{HD}$ & $0.21 \pm 3.2$& $0.17 \pm 3.3$& 		$-0.036 \pm 3.3$&	 $-0.15 \pm 3.3$&$-0.13 \pm 3.4$\\
$\tilde{C}_{ll}$ &$-0.14 \pm 0.11$&	 $-0.12 \pm 0.14$& 		$-0.10 \pm 0.16$& $-0.095 \pm 0.17$&$-0.089 \pm 0.18$\\
$\tilde{C}_{ee}$ &$-0.029 \pm 0.19$&	$-0.029 \pm 0.2$&	$-0.027 \pm 0.2$&$-0.023 \pm 0.21$& $-0.015 \pm 0.23$\\
$\tilde{C}_{eu}$ &$-27 \pm 24$&	 $-26 \pm 24$&		$-24 \pm 24$& $-22 \pm 24$& $-21 \pm 25$\\
$\tilde{C}_{ed}$ &$-27 \pm 30$&	 $-26 \pm 30$&		 $-24 \pm 31$& $-23 \pm 31$&$-21 \pm 31$\\
$\tilde{C}_{l e}$ &$-0.003 \pm 0.3$&	$-0.0053 \pm 0.3$&		$-0.0067 \pm 0.31$& $-0.0046 \pm 0.31$&$0.0037 \pm 0.32$\\
$\tilde{C}_{l u}$ &$-17 \pm 8.4$&	$-17 \pm 8.4$&		$-17 \pm 8.5$&$-17 \pm 8.5$&$-17 \pm 8.8$\\
$\tilde{C}_{l d}$ & $-32 \pm 16$& 	$-32 \pm 16$&		$-32 \pm 16$
&$-32 \pm 16$& $-31 \pm 17$\\
$\tilde{C}_{l q}^{(1)}$ & $-4 \pm 1.9$&$-3.5 \pm 2.4$&	$-2.4 \pm 3.6$&$-1.7 \pm 4.4$& $-1.1 \pm 5.8$\\
$\tilde{C}_{l q}^{(3)}$ &$-0.51 \pm 0.21$&	$-0.48 \pm 0.25$&	$-0.40 \pm 0.31$& $-0.36 \pm 0.38$&$-0.27 \pm 0.56$\\
$\tilde{C}_{qe}$ &$-1.5 \pm 26$&	$-1.8 \pm 26$&		$-2.6 \pm 26$&$-3.1 \pm 26$& $-4.1 \pm 27$\\
\hline\end{tabular}
\caption{$1 \sigma$ confidence region $\tilde{C} \pm  \sigma$ for a SMEFT error of $\{ 0\%, 0.1\%, 0.3\%, 0.5 \%, 1\% \}$ where $\tilde{C} = 100  C_{MLE}$ and $C_{MLE}$ are the MLE when a renormalizable theory is assumed to be the UV completion of the SM. \label{ConstraintsUVren}}
\end{table}

==> WNuNuMSquaredTable.tex <==

\begin{center}
\begin{table}
\tiny
\centering
\tabcolsep 8pt
\hspace*{-2.9cm}\begin{tabular}{|c|c|}
\hline
$\left(\lambda_{12}, \lambda_{34}, \lambda_{12}', \lambda_{34}' \right)$& $\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{\lambda_{12},\lambda_{34}} \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{* \lambda_{12}',\lambda_{34}'}$   \\ 
\hline \hline
$\left(0,0,0,0\right)$&$\frac{4 \left(2\pi\hat{\alpha}\right)^2\left(\bar{g}_V^{l,W}\right)^4}{s_{\that}^4  s_{12}s_{34} \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) }\left(\left(s^2-\left(s_{12}-s_{34}\right)^2\right)^2 \dfrac{4}{3} + \dfrac{64 s^2 s_{12}^2 s_{34}^2 4\left(- b + a \text{Arctanh}\left(b/a\right)\right) }{b^3} - \left(s^2 - \left(s_{12} - s_{34}\right)^2\right) \dfrac{16 s s_{12} s_{34} \left[ 2 ab + 2\left(-a^2+b^2\right)\text{Arctanh}\left(b/a\right)\right]}{b^3 }\right)$  \\
$\left(0,\pm,0,\pm\right)$&$\frac{16\left(2\pi\hat{\alpha}\right)^2 \left(\bar{g}_V^{l,W}\right)^4 s}{s_{\that}^4 2 s_{12}\lambda \left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)}\left(\left(s+s_{12}-s_{34}\right)^2 \dfrac{8}{3} + 4 s_{12}^2 \left(s- s_{12}+ s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\right)^2 \frac{4\left(ab/\left(a \pm b\right) \pm \left(\mp a + b\right) \text{Arctanh}\left(b/a\right) \right)}{b^3} \right.$ \\ &$\left.
 - 4 s_{12} \left(s + s_{12} - s_{34}\right)\left(s - s_{12} + s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right) \frac{-2b\left(a \mp 2b \right)+2\left(a\mp b\right)^2 \text{Arctanh}\left(b/a\right)}{b^3} \right) $\\
$\left(\mp,0,\mp,0\right)$&$\frac{16\left(2\pi\hat{\alpha}\right)^2 \left(\bar{g}_V^{l,W}\right)^4 s}{s_{\that}^4 2 s_{34}\lambda \left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)}\left(\left(s-s_{12}+s_{34}\right)^2 \dfrac{8}{3} + 4 s_{34}^2 \left(s + s_{12}- s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\right)^2  \frac{4\left(ab/\left(a \pm b\right) \pm \left(\mp a + b\right) \text{Arctanh}\left(b/a\right) \right)}{b^3}\right.$ \\ &$\left.
 - 4 s_{34} \left(s - s_{12} + s_{34}\right)\left(s + s_{12} - s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right) \frac{-2b\left(a \mp 2b \right)+2\left(a\mp b\right)^2 \text{Arctanh}\left(b/a\right)}{b^3}  \right)$\\
$\left(\pm,\pm,\pm,\pm \right)$&$ \frac{16 \left(2\pi\hat{\alpha}\right)^2\left(\bar{g}_V^{l,W}\right)^4}{s_{\that}^4  \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)}\left(s^2 \dfrac{4}{3}  + \left[-s\left(s_{12}+ s_{34}\right) \mp \left(s_{12}-s_{34}\right)\left(\mp s_{12} \pm s_{34} + \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right)\right]^2 \frac{4 \left(-b + a \text{Arctanh}\left(b/a\right)\right)}{b^3} \right.$ \\ &$\left. + 2 s \left[-s\left(s_{12}+ s_{34}\right)\mp \left(s_{12} -s_{34}\right)\left( \mp s_{12} \pm s_{34} + \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right)\right] \frac{2ab + 2 \left(-a^2+b^2\right) \text{Arctanh}\left(b/a\right)}{b^3}\right)$\\
$\left(\pm,\mp,\pm,\mp\right)$& $-  \frac{16 \left(2\pi\hat{\alpha}\right)^2 \left(\bar{g}_V^{l,W}\right)^4 s^2}{s_{\that}^4} \frac{4b \left(6 a^2 \pm 9 a b + 2b^2\right) \pm 12\left(\mp2a+b\right)\left(a\pm b\right)^2 \text{Arctanh}\left(b/a\right)}{3b^5}    $ \\
\hline
\end{tabular}
\caption{ \label{nu-nu}$\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{\lambda_{12},\lambda_{34}}  \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{*\lambda_{12}',\lambda_{34}'}$  for $\left(\lambda_{12},\lambda_{34},\lambda_{12}', \lambda_{34}'\right)$ leading to non zero terms of the full amplitude after integration over $\theta$. In our notations: $a=s -s_{12} - s_{34}$, $b = \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)$.}
\end{table}
\end{center}

==> WVNuMSquaredTable.tex <==
\begin{center}
\begin{table}
\tiny
\centering
\tabcolsep 8pt
\hspace*{-3cm}\begin{tabular}{|c|c|}
\hline
$\left(\lambda_{12}, \lambda_{34}, \lambda_{12}', \lambda_{34}' \right)$& $\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{* \lambda_{12},\lambda_{34}} \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{ \lambda_{12}',\lambda_{34}'}$   \\ 
\hline \hline
$\left(0,0,0,0\right)$&$\frac{-2 \left(2\pi\hat{\alpha}\right)\left(\bar{g}_V^{l,W}\right)^2 \left(\bar{F}_1^V + \bar{F}_2^V\right) \left(\bar{g}_1^V\left(s_{12}+s_{34}\right)+\bar{\kappa}_V s\right) \bar{D}^{V}\left(s\right)}{ 2 s_{\that}^2  s_{12} s_{34}  } \left[\left(s^2 - \left(s_{12} - s_{34}\right)^2\right) \frac{4}{3} - 8 s s_{12}s_{34} \frac{2 ab + 2\left(-a^2 + b^2\right)\text{Arctanh}\left(b/a\right)}{b^3} \right] $  \\
$\left(0,\pm,0,\pm\right)$&$\mp \frac{\left(2\pi\hat{\alpha}\right)\left(\bar{g}_V^{l,W}\right)^2 s \bar{D}^{V}\left(s\right)\left(\bar{g}_1^V \bar{M}_W^2 + \bar{\kappa}_V \bar{M}_W^2 + \bar{\lambda}_V s_{12}\right)}{ s_{\that}^2 s_{12} \bar{M}_W^2} \left[ \pm \left(\bar{F}_1^V + \bar{F}_2^V\right)\left(s+s_{12}-s_{34}\right) \frac{2}{3} \pm 2 \left(\bar{F}_1^V - \bar{F}_2^V\right)\left(s+s_{12}-s_{34}\right) \right.$ \\ &$ \left.+ 2  s_{12}  \left(s - s_{12} + s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right)\left(- \frac{2 \left(\bar{F}_1^V + \bar{F}_2^V \right)\left(a\mp b\right)\left(\mp b \pm a \text{Arctanh}\left(b/a\right)\right) }{b^3} \mp \left(\bar{F}_1^V - \bar{F}_2^V\right) \frac{2 \left(\pm b + \left(\mp a + b\right)\text{Arctanh}\left(b/a\right) \right)}{b^2}\right)\right]$\\
$\left(\mp,0,\mp,0\right)$&$\mp \frac{\left(2\pi\hat{\alpha}\right)\left(\bar{g}_V^{l,W}\right)^2 s \bar{D}^{V}\left(s\right)\left(\bar{g}_1^V \bar{M}_W^2 + \bar{\kappa}_V \bar{M}_W^2 + \bar{\lambda}_V s_{34}\right)}{ s_{\that}^2 s_{34} \bar{M}_W^2} \left[ \pm \left(\bar{F}_1^V + \bar{F}_2^V\right)\left(s - s_{12} + s_{34}\right) \frac{2}{3} \pm  2 \left(\bar{F}_1^V - \bar{F}_2^V\right)\left(s - s_{12} + s_{34}\right) \right.$ \\ &$ \left.+ 2  s_{34}  \left(s + s_{12} - s_{34} \pm \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right)\left(- \frac{2 \left(\bar{F}_1^V + \bar{F}_2^V\right)\left(a\mp b\right)\left(\mp b \pm a \text{Arctanh}\left(b/a\right)\right)}{b^3} \mp \left(\bar{F}_1^V - \bar{F}_2^V\right) \frac{2 \left(\pm b + \left(\mp a + b\right)\text{Arctanh}\left(b/a\right) \right)}{b^2}
\right)\right]$\\
$\left(\pm,\pm,\pm,\pm \right)$&$ - \frac{4\left(2\pi\hat{\alpha}\right)\left(\bar{g}_V^{l,W}\right)^2 \left(\bar{F}_1^V+\bar{F}_2^V\right) \left(2 \bar{g}_1^V \bar{M}_W^2 +\bar{\lambda}_V s\right) \bar{D}^{V}\left(s\right)}{2\bar{M}_W^2 s_{\that}^2 }\left[s \dfrac{4}{3} + \dfrac{\left[-s\left(s_{12}+s_{34}\right) \mp \left(s_{12} - s_{34}\right)\left(\mp s_{12} \pm s_{34} + \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \right)\right]\left[2 ab + 2 \left(-a^2+b^2\right) \text{Arctanh}\left(b/a\right)\right] }{b^3}\right]  $\\
$\left(\pm,\mp,\pm,\mp\right)$& $0$ \\
\hline
\end{tabular}
\caption{ \label{V-nu}$\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,\nu-exchange}^{\lambda_{12},\lambda_{34}}  \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{* \lambda_{12}',\lambda_{34}'}$  for $\left(\lambda_{12},\lambda_{34},\lambda_{12}', \lambda_{34}'\right)$ leading to non zero terms of the full amplitude after integration over $\theta$. In our notations: $a=s -s_{12} - s_{34}$, $b = \lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)$,$\bar{F}_1^Z = -g_{Z,eff} . g_{ZWW}. \bar{g}_L^e$, $\bar{F}_2^Z = -g_{Z,eff}. g_{ZWW} .\bar{g}_R^e$, $\bar{F}_1^{A} = \bar{F}_2^{A}=\sqrt{4\pi \hat{\alpha}}g_{AWW}$  and $\bar{D}^Z\left(s\right) = \bar{D}\left(s,\hat{m}_Z^2\right)$ and $\bar{D}^A\left(s\right) =1/s$.}
\end{table}
\end{center}


==> WVVMSquaredTable.tex <==
\begin{center}
\begin{table}
\tiny
\centering
\tabcolsep 8pt
\hspace*{-2.5cm}\begin{tabular}{|c|c|}
\hline
$\left(\lambda_{12}, \lambda_{34}, \lambda_{12}', \lambda_{34}' \right)$& $\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{\lambda_{12},\lambda_{34}} \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V'-exchange}^{* \lambda_{12}',\lambda_{34}'}$   \\ 
\hline \hline
$\left(0,0,0,0\right)$&$\frac{ \left(\bar{F}_1^V + \bar{F}_2^V\right)\left(\bar{F}_1^{V'} + \bar{F}_2^{V'}\right)\left(\bar{g}_1^V\left(s_{12}+s_{34}\right)+\bar{\kappa}_V s\right)\left(\bar{g}_1^{V'}\left(s_{12}+s_{34}\right)+\bar{\kappa}_{V'} s\right) \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \bar{D}^{V}\left(s\right) \bar{D}^{ * V'}\left(s\right)}{3 s_{12} s_{34}}$  \\
$\left(0,+,0,+\right)$,$\left(0,-,0-\right)$&$\frac{ s \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\left(\bar{F}_1^{V'}+\bar{F}_2^{V'}\right)  + 3 \left(\bar{F}_1^V -\bar{F}_2^V\right)\left(\bar{F}_1^{V'} -\bar{F}_2^{V'}\right) \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{12}\right) \left(\bar{g}_1^{V'} \bar{M}_W^2 +\bar{\kappa}_{V'} \bar{M}_W^2 +\bar{\lambda}_{V'} s_{12}\right)  \bar{D}^{V}\left(s\right)\bar{D}^{* V'}\left(s\right)}{12 s_{12}\bar{M}_W^4}$  \\
$\left(+,0,+,0\right)$, $\left(-,0,-,0\right)$&$\frac{ s \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\left(\bar{F}_1^{V'}+\bar{F}_2^{V'}\right)  + 3 \left(\bar{F}_1^V -\bar{F}_2^V\right)\left(\bar{F}_1^{V'} -\bar{F}_2^{V'}\right) \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{34}\right) \left(\bar{g}_1^{V'} \bar{M}_W^2 +\bar{\kappa}_{V'} \bar{M}_W^2 +\bar{\lambda}_{V'} s_{34}\right)  \bar{D}^{V}\left(s\right)\bar{D}^{* V'}\left(s\right)}{12 s_{34}\bar{M}_W^4}$ \\
$\left(+,+,+,+\right)$, $\left(-,-,-,-\right)$&$\frac{ \left(\bar{F}_1^V+\bar{F}_2^V\right)\left(\bar{F}_1^{V'}+\bar{F}_2^{V'}\right) \left(2 \bar{g}_1^V \bar{M}_W^2 +\bar{\lambda}_V s\right) \left(2 \bar{g}_1^{V'} \bar{M}_W^2 +\bar{\lambda}_{V'} s\right) \lambda\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right) \bar{D}^{V}\left(s\right)  \bar{D}^{*V'}\left(s\right)}{3\bar{M}_W^4}$ \\
\hline
\end{tabular}
\caption{ \label{V-V'}$\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{\lambda_{12},\lambda_{34}}  \mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{* \lambda_{12}',\lambda_{34}'}$  for $\left(\lambda_{12},\lambda_{34},\lambda_{12}', \lambda_{34}'\right)$ leading to non zero terms of the full amplitude after integration over $\theta$. In our notations: $\bar{F}_1^Z = -g_{Z,eff} . g_{ZWW}. \bar{g}_L^e$, $\bar{F}_2^Z = -g_{Z,eff}. g_{ZWW} .\bar{g}_R^e$, $\bar{F}_1^{A} = \bar{F}_2^{A}=\sqrt{4\pi \hat{\alpha}}g_{AWW}$  and $\bar{D}^Z\left(s\right) = \bar{D}\left(s,\hat{m}_Z^2\right)$ and $\bar{D}^A\left(s\right) =1/s$.}
\end{table}
\end{center}

==> WVexchangeTable.tex <==
\begin{center}
\begin{table}
\centering
\tabcolsep 8pt
\begin{tabular}{|c|c|c|}
\hline
$\lambda_{12}$ &$\lambda_{34}$& $\mathcal{M}_{e^+ e^- \rightarrow W^+ W^-,V-exchange}^{\lambda_{12},\lambda_{34}}$   \\ 
\hline \hline
$0$&$0$&$ -\frac{\left(\bar{F}_1^V + \bar{F}_2^V\right)\left(\bar{g}_1^V\left(s_{12}+s_{34}\right)+\bar{\kappa}_V s\right)\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\sin \theta \bar{D}^{V}\left(s\right)}{2\sqrt{s_{12}}\sqrt{s_{34}}}$  \\
$+$&$+$&$\frac{\left(\bar{F}_1^V+\bar{F}_2^V\right) \left(2 \bar{g}_1^V \bar{M}_W^2 +\bar{\lambda}_V s\right)\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\sin\theta \bar{D}^{V}\left(s\right)}{2\bar{M}_W^2}$\\
$-$&$-$&$\frac{\left(\bar{F}_1^V+\bar{F}_2^V\right) \left(2 \bar{g}_1^V \bar{M}_W^2 +\bar{\lambda}_V s\right)\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\sin\theta \bar{D}^{V}\left(s\right)}{2\bar{M}_W^2}$\\
$0$&$-$&$-\frac{\sqrt{s}\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\cos \theta - \bar{F}_1^V +\bar{F}_2^V \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{12}\right)\bar{D}^{V}\left(s\right)}{2\sqrt{2}\sqrt{s_{12}}\bar{M}_W^2}$ \\
$0$&$+$&$\frac{\sqrt{s}\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\cos \theta + \bar{F}_1^V -\bar{F}_2^V \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{12}\right)\bar{D}^{V}\left(s\right)}{2\sqrt{2}\sqrt{s_{12}}\bar{M}_W^2}$  \\
$+$&$0$&$\frac{\sqrt{s}\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\cos \theta - \bar{F}_1^V +\bar{F}_2^V \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{34}\right)\bar{D}^{V}\left(s\right)}{2\sqrt{2}\sqrt{s_{34}}\bar{M}_W^2}$ \\
$-$&$0$&$- \frac{\sqrt{s}\lambda^{1/2}\left(\sqrt{s},\sqrt{s_{12}},\sqrt{s_{34}}\right)\left(\left(\bar{F}_1^V+\bar{F}_2^V\right)\cos \theta + \bar{F}_1^V -\bar{F}_2^V \right) \left(\bar{g}_1^V \bar{M}_W^2 +\bar{\kappa}_V \bar{M}_W^2 +\bar{\lambda}_V s_{34}\right)\bar{D}^{V}\left(s\right)}{2\sqrt{2}\sqrt{s_{34}}\bar{M}_W^2}$  \\
$+$&$-$&$0$\\
$-$&$+$&$0$\\
\hline
\end{tabular}
\caption{ \label{V-exchange}The $W^\pm$ pair production matrix elements for $\lambda_{12},\lambda_{34}=\{0,+,-\}$ with in our notations: $\bar{F}_1^Z = -g_{Z,eff} \,  g_{ZWW} \, \bar{g}_L^e$, $\bar{F}_2^Z = -g_{Z,eff} \, g_{ZWW}  \, \bar{g}_R^e$, $\bar{F}_1^{A} = \bar{F}_2^{A}=\sqrt{4\pi \hat{\alpha}}g_{AWW}$  and $\bar{D}^Z\left(s\right) = \bar{D}\left(s,\hat{m}_Z^2\right)$ and $\bar{D}^A\left(s\right) =1/s$.}
\end{table}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> angular.tex <==
\begin{center}
\begin{table} 
\centering
\tabcolsep 2pt
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|}
\hline
- & $\frac{\delta m_w^2}{\hat{m}_w^2}$ & $\delta g_W^\nu$ & $\delta g_W^{\pm}$ & $\frac{\delta \lambda_Z}{\hat{m}_w^2}$ & $\delta \kappa_Z$ & $\delta g^1_Z$
& $\delta F^1_Z$ & $\delta F^2_Z$ & $\delta \kappa_\gamma$ & $\frac{\delta \Gamma_W}{\hat{\Gamma}_W}$  \\ 
\hline \hline
$B_1$ & -0.20 & 0.56 &  0.40  & $-9.4E^{-3}$ & $1.9E^{-2}$ & $2.0E^{-2}$ & 0.29 & $-2.5E^{-2}$ & $9.2E^{-3}$ & -0.20 \\
$B_2$ & $7.2E^{-3}$ & 0.10 &  $4.6E^{-2}$  & $1.4E^{-3}$ & $-1.9E^{-4}$ & $2.0E^{-4}$ & $-5.4E^{-3}$ & $-7.7E^{-3}$ & $-6.3E^{-4}$ & $-2.4E^{-2}$ \\
$B_3$ & $9.0E^{-3}$ & $7.0E^{-2}$ &  $2.2E^{-2}$  & $2.8E^{-3}$ & $-1.8E^{-3}$ & $-1.7E^{-3}$ & $-3.4E^{-2}$ & $-7.3E^{-3}$ & $-1.5E^{-3}$ & $-1.1E^{-2}$ \\
$B_4$ & $2.4E^{-2}$ & 0.18 &  $3.9E^{-2}$  & $9.6E^{-3}$ & $-7.6E^{-3}$ & $-7.7E^{-3}$ & -0.14 & $-1.8E^{-2}$ & $-5.4E^{-3}$ & $-9.6E^{-3}$ \\
\hline
$B_1$ & -0.13 & 0.74 &  0.52  & $-6.7E^{-3}$ & $2.5E^{-2}$ & $2.5E^{-2}$ & 0.38 & $-3.6E^{-2}$ & $1.2E^{-2}$ &-0.26 \\
$B_2$ &$1.3E^{-2}$ &$9.3E^{-2}$&  $4.2E^{-2}$  & $1.6E^{-3}$ & $-5.6E^{-4}$ & $3.6E^{-5}$ & $-1.3E^{-2}$ & $-1.1E^{-2}$ & $-1.2E^{-2}$ & $1.6E^{-3}$ \\
$B_3$ &$8.7E^{-3}$ &$7.0E^{-2}$&  $1.9E^{-2}$  & $2.5E^{-3}$ & $-2.2E^{-3}$ & $-1.9E^{-3}$ & $-4.1E^{-2}$ & $-1.0E^{-2}$ & $-2.1E^{-3}$ & $-9.6E^{-3}$ \\
$B_4$ &$2.0E^{-2}$ &0.18 &  $3.1E^{-2}$  & $8.8E^{-3}$ & $-8.7E^{-3}$ & $-8.6E^{-3}$ & -0.16 & $-2.5E^{-2}$ & $-6.7E^{-3}$ & $-1.6E^{-2}$ \\
\hline
\end{tabular}
\caption{Contributions due to the $\delta X$ in $pb$ for average $d \sigma_{CC03}/d \cos \theta$ data. The upper block of numbers is for $\sqrt{s}=188.6 \, {\rm GeV}$, the lower block of numbers is
for $\sqrt{s}=205.92 \, {\rm GeV}$. Again, the results are normalized for semi-leptonic final states.\label{angular}
$\Gamma_Z/\hat{\Gamma}_Z$ contributions are $\mathcal{O}(10^{-6})$ and not shown in the table, although they are included in the fit for completeness.}
\end{table}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> totalcrosssectionsS.tex <==
\begin{center}
\begin{table} 
\centering
\tabcolsep 4pt
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|}
\hline
$\sqrt{s}$ & $\frac{\delta m_w^2}{\hat{m}_w^2}$ & $\delta g_W^\nu$ & $\delta g_W^{\pm}$ & $\frac{\delta \lambda_Z}{\hat{m}_w^2}$ & $\delta \kappa_Z$ & $\delta g^1_Z$
& $\delta F^1_Z$ & $\delta F^2_Z$ & $\delta \kappa_\gamma$ & $\frac{\delta \Gamma_W}{\hat{\Gamma}_W}$ & $\frac{\delta \Gamma_Z}{\hat{\Gamma}_Z}$  \\ 
\hline \hline
188.6 & -2.3 & 72 &  34  & 1.3 &  -0.19 & $-7.4E^{-2}$ &  -6.6 &  -6.1 &  -0.52 & -17 & $7.1E^{-3}$\\
191.6 & -1.1 & 73 &  34  & 1.4 &  -0.22 &  $-9.2E^{-2}$ &  -7.4 &  -6.6 &  -0.58 & -17 & $7.0E^{-3}$ \\
195.5 & $-6.8E^{-2}$ & 74 &  34  & 1.4 &  -0.26 &  -0.12 &  -8.3 &  -7.1 &  -0.66 & -17 & $6.8E^{-3}$ \\
199.5 & 1.3 & 75 &  34  & 1.4 &  -0.31 &  -0.14 &  -9.2 &  -7.6 &  -0.73 & -17 & $6.5E^{-3}$\\
201.6 & 1.0 & 75 &  34  & 1.4 &  -0.33 &  -0.15 &  -9.7 &  -7.8 &  -0.77 & -17 & $6.4E^{-3}$\\
204.8 & 1.4 & 75 &  34  & 1.4  &  -0.37 &  -0.17 &  -10 &  -8.1 &  -0.82 & -17 & $6.2E^{-3}$\\
206.5 & 2.0 & 75 &  34  & 1.4  &  -0.38 &  -0.18 &  -11 &  -8.3 &  -0.85 & -17 &  $6.1E^{-3}$ \\
208.0 & 1.7 & 75 &  34  & 1.4 &  -0.40 &  -0.19 &  -11 &  -8.4 &  -0.87 & -17 &  $6.0E^{-3}$ \\
\hline
\end{tabular}
\caption{Total cross section contributions due to $\delta X$ in $pb$. Note that the results are normalized for semileptonic final states, and the $W^\pm$ decays
sensitivity is the same. To normalize to fully leptonic decays the results are divided by $4.04$. For only quark final states, the results are multiplied by $1.01$\label{crosssections}.}
\end{table}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


